SMT-Friendly Formalization of the Solidity Memory Model

Solidity is the dominant programming language for Ethereum smart contracts. This paper presents a high-level formalization of the Solidity language with a focus on the memory model. The presented formalization covers all features of the language related to managing state and memory. In addition, the formalization we provide is effective: all but few features can be encoded in the quantifier-free fragment of standard SMT theories. This enables precise and efficient reasoning about the state of smart contracts written in Solidity. The formalization is implemented in the solc-verify verifier and we provide an extensive set of tests that covers the breadth of the required semantics. We also provide an evaluation on the test set that validates the semantics and shows the novelty of the approach compared to other Solidity-level contract analysis tools.

==> ex_smtprogram.tex <==
% !TEX root = paper.tex
% !TEX program = pdflatex

\begin{figure}[htb]
\centering
\begin{subfigure}[b]{.45\linewidth}
$T(x : int, y : bool)$\\
$a : [int]T$\\
$a[0].x := 1$\\
$a[0].y := \mathit{true}$\\
$\mathit{assume}(a[1].x = 2)$
\caption{An example program.}
\end{subfigure}
\hfill
\begin{subfigure}[b]{.48\linewidth}
\todo{Declare types and consts}\\
$a_1 = a_0[0 \leftarrow T(1, a_0[0].y)]$\\
$a_2 = a_1[0 \leftarrow T(a_1[0].x, \mathit{true})]$\\
$a_2[1].x = 2$
\caption{Translation to SMT formulas.}
\end{subfigure}
\caption{An example SMT program and its translation to SMT formulas.}
\label{fig:smtprogram_ex}
\end{figure}


==> formalize_buildtree.tex <==
% !TEX root = paper.tex
% !TEX program = pdflatex

\begin{figure}[htb]
\begin{subfigure}[b]{.48\linewidth}
\centering
\begin{algorithm}[H]
	\SetAlgoLined
	\SetKwProg{Fn}{def}{:}{}
	\Fn{build(T: type)}{
		$\textit{root} := \textit{node}()$\;
		\ForEach{state variable $s$}{
			$\textit{sub} := \textit{build}(\typeof{s}, T)$\;
			\lIf{\textit{sub} $\neq$ empty}{
				add edge $\textit{root} \xrightarrow{s} \textit{sub}$%
			}
		}
		\Return{\textit{root}}
	}
	\vspace{0.5em}
	\Fn{build(S: struct type, T: type)}{
		\lIf{$S = T$}{\Return{$\textit{node}(T)$}}
		$\textit{root} := \textit{node}(S)$\;
		\ForEach{member $m_i$ of $T$}{
			$\textit{sub} := \textit{build}(\typeof{m_i}, T)$\;
			\lIf{\textit{sub} $\neq$ empty}{
				add edge $\textit{root} \xrightarrow{m_i} \textit{sub}$%
			}
		}
		\lIf{\textit{root} has subnodes}{\Return{\textit{root}}}
		\lElse{\Return{\textit{empty}}}
	}
\end{algorithm}
\end{subfigure}
\hfill
\begin{subfigure}[b]{.48\linewidth}
\centering
\begin{algorithm}[H]
	\SetAlgoLined
	\SetKwProg{Fn}{def}{:}{}
	\Fn{build(A[]: array type, T: type)}{
		\lIf{$A[] = T$}{\Return{$\textit{node}(T)$}}
		$\textit{sub} := \textit{build}(A, T)$\;
		\If{\textit{sub} $\neq$ empty}{
			$\textit{root} := \textit{node}(A[])$\;
			add edge $\textit{root} \xrightarrow{} \textit{sub}$\;
			\Return{\textit{root}}
		}
		\lElse{\Return{\textit{empty}}}
	}
	\vspace{0.5em}
	\Fn{build((K \codeintext{=>} V): mapping type, T: type)}{
		\lIf{$(K \codeintext{=>} V) = T$}{\Return{$\textit{node}(T)$}}
		$\textit{sub} := \textit{build}(V, T)$\;
		\If{\textit{sub} $\neq$ empty}{
			$\textit{root} := \textit{node}(K \codeintext{=>} V)$\;
			add edge $\textit{root} \xrightarrow{} \textit{sub}$\;
			\Return{\textit{root}}
		}
		\lElse{\Return{\textit{empty}}}
	}
\end{algorithm}
\end{subfigure}
\caption{
%
Building the storage tree for a type.\todo{Make sure indexing on edges is
consistent with examples.}
%
}
\label{fig:formalize_buildtree}
\end{figure}

